CHILES VERDES: Radio variability at an unprecedented depth and cadence in the COSMOS field

Although it is well-established that some extragalactic radio sources are time-variable, the properties of this radio variability, and its connection with host galaxy properties, remain to be explored---particularly for faint sources. Here we present an analysis of radio variable sources from the CHILES Variable and Explosive Radio Dynamic Evolution Survey (CHILES VERDES)---a partner project of the 1.4 GHz COSMOS \ion{H}{1} Large Extragalactic Survey (CHILES). CHILES VERDES provides an unprecedented combination of survey depth, duration, and cadence, with 960 hrs of 1--2 GHz continuum VLA data obtained over 209 epochs between 2013 and 2019 in a 0.44 deg$^2$ section of the well-studied extragalactic deep field, COSMOS. We identified 18 moderate-variability sources (showing $10-30\%$ flux density variation) and 40 lower variability sources (2-10$\%$ flux density variation). They are mainly active galactic nuclei (AGN) with radio luminosities in the range of $10^{22}-10^{27}$ W Hz$^{-1}$ based on cross-matching with COSMOS multi-wavelength catalogs. The moderate-variability sources span redshifts $z=0.22-1.56$, have mostly flat radio spectra ($\alpha>-0.5$), and vary on timescales ranging from days to years. Lower-variability sources have similar properties, but have generally higher radio luminosities than the moderate-variability sources, extend to $z = 2.8$, and have steeper radio spectra ($\alpha<-0.5$). No star-forming galaxy showed statistically significant variability in our analysis. The observed variability likely originates from scintillation on short ($\sim$week) timescales, and Doppler-boosted intrinsic AGN variability on long (month--year) timescales.

==> CHILES_VERDES_Variables_Final 2/affiliations.tex <==
\newcommand{\UNC}{\affiliation{Department of Physics and Astronomy, University of North Carolina at Chapel Hill, Chapel Hill, NC 27599, USA}}
\newcommand{\MSU}{\affiliation{Center for Data Intensive and Time Domain Astronomy, Department of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}}
\newcommand{\LESIA}{\affiliation{LESIA, Observatoire de Paris, CNRS, PSL, SU/UPD, Meudon, France}}
\newcommand{\USydney}{\affiliation{Sydney Institute for Astronomy, School of Physics, University of Sydney, Sydney, New South Wales 2006, Australia}}
\newcommand{\UWMad}{\affiliation{Department of Astronomy, University of Wisconsin-Madison, Madison, WI 53706, USA}}
\newcommand{\NRAO}{\affiliation{National Radio Astronomy Observatory, P.O. Box O, Socorro, NM 87801, USA}}
\newcommand{\UOxford}{\affiliation{Astrophysics, Department of Physics, University of Oxford, Keble Road, Oxford, OX1 3RH, UK}}
\newcommand{\UCapeTown}{\affiliation{Department of Astronomy, University of Cape Town, Private Bag X3, Rondenbosch, 7701, South Africa}}

==> CHILES_VERDES_Variables_Final 2/authors.tex <==
\author[0000-0002-4781-7291]{Sumit K.\ Sarbadhicary}
\MSU

\author[0000-0002-4039-6703]{Evangelia Tremou}
\LESIA

\author[0000-0001-8026-5903]{Adam J. Stewart}
\USydney

\author[0000-0002-8400-3705]{Laura Chomiuk}
\MSU 

\author[0000-0001-5826-6803]{Charee Peters}
\UWMad

\author[0000-0002-3733-2565]{Chris Hales}
\NRAO

\author[0000-0002-1468-9668]{Jay Strader}
\MSU

\author[0000-0003-3168-5922]{Emmanuel Momjian}
\NRAO

\author{Rob Fender}
\UOxford
\UCapeTown

\author{Eric M. Wilcots}
\UWMad
